Investigating the X-ray time-lags in PG 1244+026 using an extended corona model

We present an extended corona model based on ray-tracing simulations to investigate X-ray time lags in Active Galactic Nuclei (AGN). This model consists of two axial point sources illuminating an accretion disc that produce the reverberation lags. These lags are due to the time delays between the directly observed and reflection photons and are associated with the light-travel time between the source and the disc, so they allow us to probe the disc-corona geometry. We assume the variations of two X-ray sources are triggered by the same primary variations, but allow the two sources to respond in different ways (i.e. having different source responses). The variations of each source induce a delayed accretion disc response and the total lags consist of a combination of both source and disc responses. We show that the extended corona model can reproduce both the low-frequency hard and high-frequency soft (reverberation) lags. Fitting the model to the timing data of PG~1244+026 reveals the hard and soft X-ray sources at $\sim6r_{\text{g}}$ and $\sim11r_{\text{g}}$, respectively. The upper source produces small amounts of reflection and can be interpreted as a relativistic jet, or outflowing blob, whose emission is beamed away from the disc. This explains the observed lag-energy in which there is no soft lag at energies $<1$~keV as they are diluted by the soft continuum of the upper source. Finally, our models suggest that the fluctuations propagating between the two sources of PG~1244+026 are possible but only at near the speed of light.

==> shortcuts.tex <==
\newcommand\aj{{AJ}}%
          % Astronomical Journal
\newcommand\actaa{{Acta Astron.}}%
  % Acta Astronomica
\newcommand\araa{{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{{BAAS}}%
          % Bulletin of the AAS
\newcommand\caa{{Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{{Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{{Icarus}}%
  % Icarus
\newcommand\jcap{{J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\na{{New A}}%
  % New Astronomy
\newcommand\nar{{New A Rev.}}%
  % New Astronomy Review
\newcommand\pra{{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasa{{PASA}}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{{PASP}}%
          % Publications of the ASP
\newcommand\pasj{{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{{Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{{Nature}}%
          % Nature
\newcommand\iaucirc{{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{{Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{{J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{{Proc.~SPIE}}%
          % Proceedings of the SPIE
